Probing Brain Context-Sensitivity with Masked-Attention Generation

Two fundamental questions in neurolinguistics concerns the brain regions that integrate information beyond the lexical level, and the size of their window of integration. To address these questions we introduce a new approach named masked-attention generation. It uses GPT-2 transformers to generate word embeddings that capture a fixed amount of contextual information. We then tested whether these embeddings could predict fMRI brain activity in humans listening to naturalistic text. The results showed that most of the cortex within the language network is sensitive to contextual information, and that the right hemisphere is more sensitive to longer contexts than the left. Masked-attention generation supports previous analyses of context-sensitivity in the brain, and complements them by quantifying the window size of context integration per voxel.

==> guidelines.tex <==
<5 MB (megabytes) in size. 
 To request an exception, contact the paper submission technical support at: papers@ccneuro.org.

The filename of the document file should be the first author's last name, followed by the appropriate extension (.pdf). For example, if the first author's name is Jane Smith, you would submit your file as "smith.pdf". The paper submission process will append the filename with a unique identifier when it is stored on our system, so multiple submissions with the same name will not overwrite each other and will be distinguishable.



To submit your document and author information, go to the 'Submit a Paper' link in the 'Program Information" menu on the CCN 2023 homepage: https://2023.ccneuro.org/.
